Synthesizing Safe and Efficient Kernel Extensions for Packet Processing

Extended Berkeley Packet Filter (BPF) has emerged as a powerful method to extend packet-processing functionality in the Linux operating system. BPF allows users to write code in high-level languages (like C or Rust) and execute them at specific hooks in the kernel, such as the network device driver. To ensure safe execution of a user-developed BPF program in kernel context, Linux uses an in-kernel static checker. The checker allows a program to execute only if it can prove that the program is crash-free, always accesses memory within safe bounds, and avoids leaking kernel data. BPF programming is not easy. One, even modest-sized BPF programs are deemed too large to analyze and rejected by the kernel checker. Two, the kernel checker may incorrectly determine that a BPF program exhibits unsafe behaviors. Three, even small performance optimizations to BPF code (e.g., 5% gains) must be meticulously hand-crafted by expert developers. Traditional optimizing compilers for BPF are often inadequate since the kernel checker's safety constraints are incompatible with rule-based optimizations. We present K2, a program-synthesis-based compiler that automatically optimizes BPF bytecode with formal correctness and safety guarantees. K2 produces code with 6--26% reduced size, 1.36%--55.03% lower average packet-processing latency, and 0--4.75% higher throughput (packets per second per core) relative to the best clang-compiled program, across benchmarks drawn from Cilium, Facebook, and the Linux kernel. K2 incorporates several domain-specific techniques to make synthesis practical by accelerating equivalence-checking of BPF programs by 6 orders of magnitude.

==> eval-latency-harness.tex <==
\begin{table*}[!t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Program & -O1 (ns) & -O2 (ns) & Superopt (ns) & Superopt v2 (ns)\\ \hline
cilium from-network & 79.9 & 78.7 & 72.3 & 68.8 \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of execution runtimes for programs compiled with Clang using -O1 and -O2 along with Superopt. These latencies were calculated by running each program for 100,00 iterations, subtracting the base running time from each result, and taking the mean of the distribution.}
\end{table*}


==> eval-profiled-instruction-latencies.tex <==
\begin{table}[!t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Instruction & Average runtime (ns)\\ \hline
ADD32XC & 0.9 \\ \hline
MUL32XC & 4.5 \\ \hline
DIV32XC & 25 \\ \hline
MOD32XC & 14.1 \\ \hline
JEQ32XC & 2.1 \\ \hline
JNE32XC & 4.7 \\ \hline
STXDW & 0.9 \\ \hline
LDXDW & 0.5 \\ \hline
XADD32 & 17 \\ \hline
BE64 & 0.9 \\ \hline
BPF\_FUNC\_map\_lookup\_elem & 2.5 \\ \hline
BPF\_FUNC\_map\_update\_elem & 74.6 \\ \hline

\end{tabular}
\end{center}
\caption{Comparison of estimated BPF instruction latencies after benchmarking. For each instruction we generated a program that executed the instruction 250 -- 1000 consecutive times. We executed this program 1000 times and recorded each result. For each result, we subtracted the base running time and divided it by 1000. Lastly, we took the mean of the entire distribution.}
\end{table}

